Generalized Stability Approach for Regularized Graphical Models

Selecting regularization parameters in penalized high-dimensional graphical models in a principled, data-driven, and computationally efficient manner continues to be one of the key challenges in high-dimensional statistics. We present substantial computational gains and conceptual generalizations of the Stability Approach to Regularization Selection (StARS), a state-of-the-art graphical model selection scheme. Using properties of the Poisson-Binomial distribution and convex non-asymptotic distributional modeling we propose lower and upper bounds on the StARS graph regularization path which results in greatly reduced computational cost without compromising regularization selection. We also generalize the StARS criterion from single edge to induced subgraph (graphlet) stability. We show that simultaneously requiring edge and graphlet stability leads to superior graph recovery performance independent of graph topology. These novel insights render Gaussian graphical model selection a routine task on standard multi-core computers.

==> Notation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%        Packages                   %%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[ansinew]{inputenc}
%\usepackage{graphics} 
\usepackage{graphicx}
\usepackage{color} 
\usepackage{textcomp} 
\usepackage{amsfonts} 
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{latexsym}
%\usepackage{caption}
\usepackage{array}
\usepackage{float}
\usepackage{amsthm} 
\usepackage{calc}
\usepackage{perpage}
\usepackage{textcomp}
\usepackage{verbatim} 
\usepackage{marvosym}
\usepackage{hieroglf}
\usepackage{multirow} % can combine rows and columns of tables
\usepackage{rotating} % Can rotate text, can be combined with multirow
% to write vertical text in tables
%\usepackage{epstopdf}
\usepackage{dsfont} %for nice indicator
\usepackage{grffile} %to include graphics paths
\usepackage{enumitem}

\usepackage[english]{babel}

\usepackage{tikz}

\usepackage[ruled]{algorithm2e} % For Algorithms

% change the layout of the algorithms as do options boxed, boxruled, ruled and algoruled


%\usepackage{geometry}
%\usepackage{amsfonts}
%\usepackage{dsfont}
%\usepackage[latin1]{inputenc}
%\usepackage{amssymb , amsmath, amsthm, amsopn, amstext, amscd}
%\usepackage[T1]{fontenc}
%\usepackage{latexsym, enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%        Writing                  %%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\etal}{{\it et al.}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%        Theorems                   %%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{definition}{Definition}[section]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%        Revisions/Reviews          %%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\quotejl}[1]{\begin{quote}{\it ``#1"} \end{quote}}
\newcommand{\tot}{$\to$} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%        Working in Groups          %%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\todo}[1]{\marginpar{\textcolor{red}{\flushleft\tiny #1}}} 


\usepackage[textwidth=1cm, textsize=footnotesize]{todonotes}


\newcommand{\yoyo}[1]{\todo[color=blue!20]{{\bf Johannes:} #1}}
\newcommand{\another}[1]{\todo[color=cyan!20]{{\bf Another:} #1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%        Mathematics                %%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%sign
\DeclareMathOperator*{\sign}{sign}


% Indicator
\newcommand{\1}{{\rm 1}\mskip -4,5mu{\rm l} }


% Argmin and argmax
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}

% Argmin
%\newcommand{\argmin}{\mathop{\mathrm{arg\,min}}}


% Norm
\newcommand{\norm}[2][]{{\left \lVert #2 \right\rVert}_{#1}}

% Operatorname
\newcommand{\op}[1]{\operatorname{#1}}  % Lettre droite!!!!


% To the power -1
\newcommand{\pmo}{^{\text -1}}

% SETS
\def\A{\mathbb{A}}
\def\B{\mathbb{B}}
\def\C{\mathbb{C}}
\def\D{\mathbb{D}}
\def\E{\mathbb{E}}
\def\F{\mathbb{F}}
\def\G{\mathbb{G}}
\def\I{\mathbb{I}}

\def\L{\mathbb{L}}

\def\N{\mathbb{N}}

\def\R{\mathbb{R}}

\def\T{\mathbb{T}}

\def\Z{\mathbb{Z}}

\def\Cc{\mathcal{C}}

\newcommand{\rp}{\mathbb{R}^p}
\newcommand{\rn}{\mathbb{R}^n}
\newcommand{\rnp}{\mathbb{R}^{n\times p}}
\newcommand{\rpp}{\mathbb{R}^{p\times p}}
\newcommand{\otp}{\{1,\dots,p\}}
\newcommand{\otn}{\{1,\dots,n\}}

% Probabilities
\newcommand{\mpr}{\mathbb{P}}
\newcommand{\mprn}{\mathbb{P}_n}
\def\Var{\mathbb{V}\mbox{ar}\,}
\def\vt{\mbox{Var}_\theta\,}
\def\cov{\mbox{Cov}\,}
\def\ct{\mbox{Cov}_\theta\,}


% Sums
\newcommand{\si}{\sum_{i=1}^n}
\def\sino{\frac{1}{n}\sum_{i=1}^n}

% Lasso and SQRT Lasso
\newcommand{\be}{\widehat\beta}
\newcommand{\set}{\widehat S}
\newcommand{\setnor}{{|\widehat S|}}
\newcommand{\estset}{\widehat\beta_{\widehat S}}
\newcommand{\matset}{X_{\widehat S}}
\newcommand{\graset}{X_{\widehat S}^TX_{\widehat S}}
\newcommand{\rset}{R^{\setnor}}
\newcommand{\bt}{\beta^*}

% Refitting
\newcommand{\estref}{\overline{\beta}}
\newcommand{\setref}{\overline S}

